Fixed Parameter Approximation Scheme for Min-max $k$-cut

We consider the graph $k$-partitioning problem under the min-max objective, termed as Minmax $k$-cut. The input here is a graph $G=(V,E)$ with non-negative edge weights $w:E\rightarrow \mathbb{R}_+$ and an integer $k\geq 2$ and the goal is to partition the vertices into $k$ non-empty parts $V_1, \ldots, V_k$ so as to minimize $\max_{i=1}^k w(\delta(V_i))$. Although minimizing the sum objective $\sum_{i=1}^k w(\delta(V_i))$, termed as Minsum $k$-cut, has been studied extensively in the literature, very little is known about minimizing the max objective. We initiate the study of Minmax $k$-cut by showing that it is NP-hard and W[1]-hard when parameterized by $k$, and design a parameterized approximation scheme when parameterized by $k$. The main ingredient of our parameterized approximation scheme is an exact algorithm for Minmax $k$-cut that runs in time $(\lambda k)^{O(k^2)}n^{O(1)}$, where $\lambda$ is value of the optimum and $n$ is the number of vertices. Our algorithmic technique builds on the technique of Lokshtanov, Saurabh, and Surianarayanan (FOCS, 2020) who showed a similar result for Minsum $k$-cut. Our algorithmic techniques are more general and can be used to obtain parameterized approximation schemes for minimizing $\ell_p$-norm measures of $k$-partitioning for every $p\geq 1$.

==> hardness-densest-k-set.tex <==
\section{NP-hardness}
\label{sec:hardness}
\begin{theorem}\label{thm np hardness}
\mmkc is strongly NP-hard and W[1]-hard.
\end{theorem}
\begin{proof}
We will show a reduction from \textsc{Densest $k$-subset} \knote{\textsc{$r$-clique}?} in the unweighted case. \knote{Define this problem and state the known hardness results for this problem.} 

\knote{Use notation consistent with introduction.}

Let $(G=(V,E),h)$ be an instance of \textsc{Densest $k$-subset}, where $V=\{v_1,\ldots,v_n\}$. \knote{Let $M=...$ and $N=...$.}
We define a graph $G'=(V',E')$ as following.
\begin{align*}
    V'=&\{u_{i,j}:i\in[n],j\in[N]\}\sqcup\{w_j:j\in[N]\},
    \\E'=&\{u_{i,j}u_{i,j'}:i\in[n],j,j'\in[N]\}\sqcup\{u_{i,1}u_{i',1}:i,i'\in[n],v_iv_{i'}\in E\}
    \\&\sqcup\{w_jw_{j'}:j,j'\in [N]\}\sqcup\{u_{i,j}w_j:i\in[n],j\in[M-\deg_G(v_i)]\}.
\end{align*}
Here $M=\max\{(n+1)^2,3m\}$ and $N=Mn+2$ \knote{Remove this. Also, use $\cup$ above. An example figure would be helpful here. }. 
Alternatively, we can think of $G'$ to be constructed as follows. Each vertex $v_i\in V$ induces an $N$-clique $\{u_{i,j}:j\in[N]\}$ in $G'$. 
Each edge $e=v_iv_{i'}\in E$ induces an edge $u_{i,1}u_{i',1}$ between the two corresponding $N$-cliques in $G'$. 
Moreover, an additional $N$-clique $\{w_j\in j\in[N]\}$ is added. 
For each $v_i\in V$, we add $M-\deg_G(v_i)$ edges to connect the $N$-clique induced by $v_i$ and the additional $N$-clique.

We claim that on instance $(G',w,h+1)$, where $w$ is uniformly 1, \mmkc yields a partition $\mathcal{P}=(P_1,\ldots,P_{h+1})$ such that for all $\ell\in[h]$, we have $P_\ell=\{u_{i_l,j}:j\in[N]\}$ for some $i_\ell$ and $\{v_{i_1},\ldots,v_{i_h}\}$ is a densest $h$-subset of $G$.

Let $V_0\subseteq V$ be a densest $h$-subset of $V$. 
Without loss of generality, let $V_0=\{v_1,\ldots,v_h\}$. 
Consider the partition $\mathcal{Q}=\{Q_1,\ldots,Q_{h+1}\}$ given by
\begin{align*}
    Q_i&=\{u_{i,j}:j\in[N]\},\,\forall i\in[h],
    \\Q_{h+1}&=V'\backslash(Q_1\cup\ldots\cup Q_h).
\end{align*}
Here
\begin{align*}
    |\delta_{G'}(Q_i)|&=(M-\deg_G(v_i))+\deg_G(v_i)=M,\,\forall i\in[h],
    \\|\delta_{G'}(Q_{h+1})|&=\sum_{v\in V_0}(M-\deg_G(v))+|E[V_0,V\backslash V_0]|
    \\&=\sum_{v\in V_0}(M-\deg_G(v))+\sum_{v\in V_0}\deg_G(v)-2|E[V_0]|
    \\&=Mh-2|E[V_0]|.
\end{align*}
By choice of $M$, the objective value for $\mathcal{Q}$ is $Mh-2|E[V_0]|$. 
An $(h+1)$-cut that separates a $N$-clique results in objective value at least $N-1>Mh-2|E[V_0]|$, and hence no optimum $(h+1)$-cut separates $N$-cliques.
Therefore, it is equivalent to consider optimum $(h+1)$-cut in the following weighted graph $G''=(V'',E'')$ whose cost function is $w''$:
\begin{align*}
    V''&=V\sqcup\{w\},
    \\E''&=E\sqcup \{wv:v\in V\},
    \\w''(e)&=1,\,\forall e\in E,
    \\w''(wv)&=M-\deg_G(v),\,\forall v\in V.
\end{align*}
$G''$ can be obtained from $G'$ by contracting each of the $n+1$ $N$-cliques in $G'$.
Now we fix $\mathcal{R}=(R_1,\ldots,R_{h+1})$ to be an optimum $(h+1)$-cut of $G''$, where $w\in R_{h+1}$. 
Projecting $\mathcal{Q}$ onto $G''$ yields a feasible $(h+1)$-cut with objective value $Mh-2|E[V_0]|$, which implies $\max_{i\in[h+1]}w''(\delta_{G''}(R_i))\leq Mh-2|E[V_0]|$. 
It follows that
\begin{align*}
    Mh-2|E[V_0]|\geq w''(\delta_{G''}(R_{h+1}))\geq \sum_{v\in R_1\cup\ldots\cup R_h}(M-\deg_G(v))\geq (M-n)|R_1\cup\ldots\cup R_h|
\end{align*}
and this forces $|R_1\cup\ldots\cup R_h|\leq h$ by choice of $M$. 
Moreover, this implies $R_1,\ldots,R_h$ are all singleton sets. 
This allows us to write $R_\ell=\{v_{i_\ell}\}$ for some $i_\ell\in[n]$ for each $\ell\in[h]$.

The cut values of $R_1,\ldots,R_{h+1}$ are given by
\begin{align*}
    w''(\delta_{G''}(R_\ell))&=M-\deg_G(v_{i_\ell})+\deg_G(v_{i_\ell})=M,\,\forall \ell\in[h],
    \\w''(\delta_{G''}(R_{h+1}))&=\sum_{v\in R_1\cup\ldots\cup R_h}(M-\deg_G(v))+c''(E[R_1\cup\ldots\cup R_h,V\backslash(R_1\cup\ldots\cup R_h)])
    \\&=\sum_{v\in R_1\cup\ldots\cup R_h}(M-\deg_G(v))+\sum_{v\in R_1\cup\ldots\cup R_h}\deg_G(v)-2|E[R_1\cup\ldots\cup R_h]|
    \\&=Mh-2|E[R_1\cup\ldots\cup R_h]|.
\end{align*}
The objective value of $\mathcal{R}$ is then $Mh-2|E[R_1\cup\ldots\cup R_h]|$. 
The partition obtained from projecting $\mathcal{Q}$ onto $G''$ has objective value $Mh-2|E[V_0]|$, so we know that
\[Mh-2|E[R_1\cup\ldots\cup R_h]|\leq Mh-2|E[V_0]|.\]
This implies $|E[R_1\cup\ldots\cup R_h]|\geq |E[V_0]|$, which means $R_1\cup\ldots\cup R_h=\{v_{i_1},\ldots,v_{i_h}\}$ is a densest $h$-subset. 
Lifting $\mathcal{R}$ back to $G'$, we obtain a $(h+1)$-cut $\mathcal{P}=(P_1,\ldots,P_{h+1})$ such that $P_l=\{u_{i_l,j}:j\in[N]\}$ and $\{v_{i_1},\ldots,v_{i_h}\}$ is a densest $h$-subset of $G$. 
Our claim is proved.

The graph $G'$ has size $\poly(n)$. This shows \mmkc is indeed strongly NP-hard and W[1]-hard.
\end{proof}
